Optimality and stability of the radial shapes for the Sobolev trace constant

In this work we establish the optimality and the stability of the ball for the Sobolev trace operator $W^{1,p}(\Omega)\hookrightarrow L^q(\partial\Omega)$ among convex sets of prescribed perimeter for any $1< p <+\infty$ and $1\le q\le p$. More precisely, we prove that the trace constant $\sigma_{p,q}$ is maximal for the ball and the deficit is estimated from below by the Hausdorff asymmetry. With similar arguments, we prove the optimality and the stability of the spherical shell for the Sobolev exterior trace operator $W^{1,p}(\Omega_0\setminus\overline{\Theta})\hookrightarrow L^q(\partial\Omega_0)$ among open sets obtained removing from a convex set $\Omega_0$ a suitably smooth open hole $\Theta\subset\subset\Omega_0$, with $\Omega_0\setminus\overline{\Theta}$ satisfying a volume and an outer perimeter constraint.

==> bibliography.tex <==
@article {MarRossi,
    AUTHOR = {Mart\'inez, Sandra and Rossi, Julio D.},
     TITLE = {Isolation and simplicity for the first eigenvalue of the
              {$p$}-{L}aplacian with a nonlinear boundary condition},
   JOURNAL = {Abstr. Appl. Anal.},
  FJOURNAL = {Abstract and Applied Analysis},
    VOLUME = {7},
      YEAR = {2002},
    NUMBER = {5},
     PAGES = {287--293},
      ISSN = {1085-3375,1687-0409},
   MRCLASS = {35P30 (35J60 35J65)},
  MRNUMBER = {1908191},
MRREVIEWER = {Raffaele\ Chiappinelli},
       DOI = {10.1155/S108533750200088X},
       URL = {https://doi.org/10.1155/S108533750200088X},
}

@article{cpp,
AUTHOR = {Cito, Simone and Paoli, Gloria and Piscitelli, Gianpaolo},
     TITLE = {A stability result for the first {R}obin-{N}eumann eigenvalue:
              a double perturbation approach},
   JOURNAL = {Commun. Contemp. Math.},
  FJOURNAL = {Communications in Contemporary Mathematics},
    VOLUME = {27},
      YEAR = {2025},
    NUMBER = {6},
     PAGES = {Paper No. 2450039, 35},
      ISSN = {0219-1997,1793-6683},
   MRCLASS = {35P15 (35B35 35J25 49Q10 49R05)},
  MRNUMBER = {4911886},
       DOI = {10.1142/S0219199724500391},
       URL = {https://doi.org/10.1142/S0219199724500391},
}



          
@article {giorgi1,
    AUTHOR = {Giorgi, Tiziana and Smits, Robert},
     TITLE = {Eigenvalue estimates and critical temperature in zero fields
              for enhanced surface superconductivity},
   JOURNAL = {Z. Angew. Math. Phys.},
  FJOURNAL = {Zeitschrift f\"{u}r Angewandte Mathematik und Physik. ZAMP.
              Journal of Applied Mathematics and Physics. Journal de
              Math\'{e}matiques et de Physique Appliqu\'{e}es},
    VOLUME = {58},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {224--245},
      ISSN = {0044-2275},
   MRCLASS = {82D55 (35J25 35P15 60J65 82C41)},
  MRNUMBER = {2305713},
MRREVIEWER = {Lia Bronsard},
       DOI = {10.1007/s00033-005-0049-y},
       URL = {https://doi.org/10.1007/s00033-005-0049-y},
}


@article {sabina,
    AUTHOR = {Lacey, A. A. and Ockendon, J. R. and Sabina, J.},
     TITLE = {Multidimensional reaction diffusion equations with nonlinear
              boundary conditions},
   JOURNAL = {SIAM J. Appl. Math.},
  FJOURNAL = {SIAM Journal on Applied Mathematics},
    VOLUME = {58},
      YEAR = {1998},
    NUMBER = {5},
     PAGES = {1622--1647},
      ISSN = {0036-1399},
   MRCLASS = {35K57 (35C20 41A60)},
  MRNUMBER = {1637882},
MRREVIEWER = {Si Ning Zheng},
       DOI = {10.1137/S0036139996308121},
       URL = {https://doi.org/10.1137/S0036139996308121},
}

@article {lemenant,
    AUTHOR = {Lemenant, Antoine and Mainini, Edoardo},
     TITLE = {On convex sets that minimize the average distance},
   JOURNAL = {ESAIM Control Optim. Calc. Var.},
  FJOURNAL = {ESAIM. Control, Optimisation and Calculus of Variations},
    VOLUME = {18},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {1049--1072},
      ISSN = {1292-8119},
   MRCLASS = {49Q10 (49K30)},
  MRNUMBER = {3019472},
MRREVIEWER = {Georg S. Weiss},
       DOI = {10.1051/cocv/2011190},
       URL = {https://doi.org/10.1051/cocv/2011190},
}

@article{paoli2020sharp,
  AUTHOR = {Paoli, Gloria and Piscitelli, Gianpaolo and Trani, Leonardo},
     TITLE = {Sharp estimates for the first {$p$}-{L}aplacian eigenvalue and
              for the {$p$}-torsional rigidity on convex sets with holes},
   JOURNAL = {ESAIM Control Optim. Calc. Var.},
  FJOURNAL = {ESAIM. Control, Optimisation and Calculus of Variations},
    VOLUME = {26},
      YEAR = {2020},
     PAGES = {Paper No. 111, 15},
      ISSN = {1292-8119,1262-3377},
   MRCLASS = {35J25 (35J92 35P15 47J30)},
  MRNUMBER = {4185065},
       DOI = {10.1051/cocv/2020033},
       URL = {https://doi.org/10.1051/cocv/2020033},
}

@article{amos1974computation,
  title={Computation of modified {B}essel functions and their ratios},
  author={Amos, Donald E},
  journal={Mathematics of computation},
  volume={28},
  number={125},
  pages={239--251},
  year={1974}
}

@article{bbg,
 AUTHOR = {Bogosel, B. and Bucur, D. and Giacomini, A.},
     TITLE = {Optimal shapes maximizing the {S}teklov eigenvalues},
   JOURNAL = {SIAM J. Math. Anal.},
  FJOURNAL = {SIAM Journal on Mathematical Analysis},
    VOLUME = {49},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {1645--1680},
      ISSN = {0036-1410,1095-7154},
   MRCLASS = {49J35 (26A45 49J45 58C40)},
  MRNUMBER = {3640624},
MRREVIEWER = {Giles\ Auchmuty},
       DOI = {10.1137/16M1075260},
       URL = {https://doi.org/10.1137/16M1075260},
}

@article{bucur2016robin,
  title={The {R}obin--{L}aplacian problem on varying domains},
  author={Bucur, Dorin and Giacomini, Alessandro and Trebeschi, Paola},
  journal={Calculus of Variations and Partial Differential Equations},
  volume={55},
  number={6},
  pages={1--29},
  year={2016},
  publisher={Springer}
}

@article{bucurcito,
     AUTHOR = {Bucur, Dorin and Cito, Simone},
     TITLE = {Geometric control of the {R}obin {L}aplacian eigenvalues: the
              case of negative boundary parameter},
   JOURNAL = {J. Geom. Anal.},
  FJOURNAL = {Journal of Geometric Analysis},
    VOLUME = {30},
      YEAR = {2020},
    NUMBER = {4},
     PAGES = {4356--4385},
      ISSN = {1050-6926,1559-002X},
   MRCLASS = {49Q10 (31C45 35J05 35P15 49R05)},
  MRNUMBER = {4167286},
MRREVIEWER = {Nunzia\ Gavitone},
       DOI = {10.1007/s12220-019-00245-9},
       URL = {https://doi.org/10.1007/s12220-019-00245-9},
}

@article{citoconvex,
  title={{Existence and Regularity of Optimal Convex Shapes for Functionals Involving the {R}obin Eigenvalues}},
  author={S. Cito},
  journal={Journal of Convex Analysis},
  volume={26},
  number={3},
  pages={925--943},
  year={2019},
  publisher={HELDERMANN VERLAG LANGER GRABEN 17, 32657 LEMGO, GERMANY}
}

@article{egert2017characterizations,
  title={Characterizations of {S}obolev functions that vanish on a part of the boundary},
  author={Egert, Moritz and Tolksdorf, Patrick},
  journal={Discrete \& Continuous Dynamical Systems-S},
  volume={10},
  number={4},
  pages={729},
  year={2017},
  publisher={American Institute of Mathematical Sciences}
}


@book{schneider2014convex,
  title={Convex Bodies: The {B}runn--{M}inkowski Theory},
  author={Schneider, Rolf},
  volume={151},
  year={2013},
  publisher={Cambridge University Press}
}


@article{henrot2019optimizing,
  title={Optimizing the first {D}irichlet eigenvalue of the {L}aplacian with an obstacle},
  author={Henrot, Antoine and Zucco, Davide},
  journal={Annali della Scuola Normale Superiore di Pisa-Classe di Scienze},
  volume={19},
  pages={1535--1559},
  year={2019}
}

@article{van2006anisotropic,
  title={Anisotropic symmetrization},
  author={Van Schaftingen, Jean},
  journal={Annales de l'IHP Analyse non lin{\'e}aire},
  volume={23},
  number={4},
  pages={539--565},
  year={2006}
}

@book{abramowitz2006handbook,
  title={Handbook of mathematical functions with formulas, graphs, and mathematical tables},
  author={Abramowitz, Milton and Stegun, Irene A},
  publisher={Washington: US Govt. Print},
  year={2006}
}

@article{gazzola1999existence,
  AUTHOR = {Gazzola, Filippo},
     TITLE = {Existence of minima for nonconvex functionals in spaces of
              functions depending on the distance from the boundary},
   JOURNAL = {Arch. Ration. Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {150},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {57--75},
      ISSN = {0003-9527,1432-0673},
   MRCLASS = {49J45 (49M99 49Q99)},
  MRNUMBER = {1738167},
MRREVIEWER = {Bianca\ Stroffolini},
       DOI = {10.1007/s002050050180},
       URL = {https://doi.org/10.1007/s002050050180},
}

@article{brandolini2010upper,
 AUTHOR = {Brandolini, Barbara and Nitsch, Carlo and Trombetti, Cristina},
     TITLE = {An upper bound for nonlinear eigenvalues on convex domains by
              means of the isoperimetric deficit},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {94},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {391--400},
      ISSN = {0003-889X,1420-8938},
   MRCLASS = {35P05 (35J10)},
  MRNUMBER = {2643973},
MRREVIEWER = {Antonio\ Su\'arez Fern\'andez},
       DOI = {10.1007/s00013-010-0102-8},
       URL = {https://doi.org/10.1007/s00013-010-0102-8},
}


@article{payne1961some,
  AUTHOR = {Payne, L. E. and Weinberger, H. F.},
     TITLE = {Some isoperimetric inequalities for membrane frequencies and
              torsional rigidity},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {2},
      YEAR = {1961},
     PAGES = {210--216},
      ISSN = {0022-247X},
   MRCLASS = {73.53},
  MRNUMBER = {149735},
MRREVIEWER = {R.\ Zurm\"uhl},
       DOI = {10.1016/0022-247X(61)90031-2},
       URL = {https://doi.org/10.1016/0022-247X(61)90031-2},
}

@incollection{hersch1962contribution,
  AUTHOR = {Hersch, Joseph},
     TITLE = {Contribution to the method of interior parallels applied to
              vibrating membranes},
 BOOKTITLE = {Studies in mathematical analysis and related topics},
    SERIES = {Stanford Studies in Mathematics and Statistics},
    VOLUME = {IV},
     PAGES = {132--139},
 PUBLISHER = {Stanford Univ. Press, Stanford, CA},
      YEAR = {1962},
   MRCLASS = {73.35},
  MRNUMBER = {163492},
MRREVIEWER = {H.\ F.\ Weinberger},
}

@article{weinberger1963effectless,
  title={An effectless cutting of a vibrating membrane},
  author={Weinberger, Hans},
  journal={Pacific Journal of Mathematics},
  volume={13},
  number={4},
  pages={1239--1240},
  year={1963},
  publisher={Mathematical Sciences Publishers}
}

@article{anoop2020reverse,
  title={On reverse {F}aber-{K}rahn inequalities},
  author={Anoop, TV and Kumar, K Ashok},
  journal={Journal of Mathematical Analysis and Applications},
  volume={485},
  number={1},
  pages={123766},
  year={2020},
  publisher={Elsevier}
}


@article{zaremba1910probleme,
  title={Sur un probleme mixte relatif a l'{\'e}quation de {L}aplace},
  author={Zaremba, S},
  journal={Bulletin de l’Acad{\'e}mie des sciences de Cracovie. Classe des sciences math{\'e}matiques et naturelles. S{\'e}rie A},
  pages={313--344},
  year={1910}
}


@article{crasta2002sharp,
  title={A Sharp Upper Bound for the Torsional Rigidity of Rods by Means of Web Functions},
  author={Crasta, Graziano and Fragal{\`a}, Ilaria and Gazzola, Filippo},
  journal={Archive for rational mechanics and analysis},
  volume={164},
  number={3},
  pages={189--211},
  year={2002},
  publisher={Springer}
}

@book{bucur2004variational,
 AUTHOR = {Bucur, Dorin and Buttazzo, Giuseppe},
     TITLE = {Variational methods in shape optimization problems},
    SERIES = {Progress in Nonlinear Differential Equations and their
              Applications},
    VOLUME = {65},
 PUBLISHER = {Birkh\"auser Boston, Inc., Boston, MA},
      YEAR = {2005},
     PAGES = {viii+216},
      ISBN = {978-0-8176-4359-1; 0-8176-4359-1},
   MRCLASS = {49-02 (49Q10 49Q15 74P99 74Q99)},
  MRNUMBER = {2150214},
MRREVIEWER = {Jan\ Soko\l owski},
}

@article{cochran1967monotonicity,
  title={The monotonicity of modified {B}essel functions with respect to their order},
  author={Cochran, James Alan},
  journal={Journal of Mathematics and Physics},
  volume={46},
  number={1-4},
  pages={220--222},
  year={1967},
  publisher={Wiley Online Library}
}


@article{dellapietra2020optimal,
 AUTHOR = {Della Pietra, Francesco and Piscitelli, Gianpaolo},
     TITLE = {An optimal bound for nonlinear eigenvalues and torsional
              rigidity on domains with holes},
   JOURNAL = {Milan J. Math.},
  FJOURNAL = {Milan Journal of Mathematics},
    VOLUME = {88},
      YEAR = {2020},
    NUMBER = {2},
     PAGES = {373--384},
      ISSN = {1424-9286,1424-9294},
   MRCLASS = {35P15 (35J25 35J92 47J30)},
  MRNUMBER = {4182078},
       DOI = {10.1007/s00032-020-00320-9},
       URL = {https://doi.org/10.1007/s00032-020-00320-9},
}


@article{anoop2023domain,
AUTHOR = {Anoop, T. V. and Ashok Kumar, K.},
     TITLE = {Domain variations of the first eigenvalue via a strict
              {F}aber-{K}rahn type inequality},
   JOURNAL = {Adv. Differential Equations},
  FJOURNAL = {Advances in Differential Equations},
    VOLUME = {28},
      YEAR = {2023},
    NUMBER = {7-8},
     PAGES = {537--568},
      ISSN = {1079-9389},
   MRCLASS = {35P15 (35J92 47J10 49Q10 49R05)},
  MRNUMBER = {4577002},
       DOI = {10.57262/ade028-0708-537},
       URL = {https://doi.org/10.57262/ade028-0708-537},
}  



@article{anoop2021shape,
  AUTHOR = {Anoop, T. V. and Ashok Kumar, K. and Kesavan, S.},
     TITLE = {A shape variation result via the geometry of eigenfunctions},
   JOURNAL = {J. Differential Equations},
  FJOURNAL = {Journal of Differential Equations},
    VOLUME = {298},
      YEAR = {2021},
     PAGES = {430--462},
      ISSN = {0022-0396,1090-2732},
   MRCLASS = {35B06 (35B07 35B50 35B51 35Q93 49Q10 49Q12 58J70)},
  MRNUMBER = {4288249},
       DOI = {10.1016/j.jde.2021.07.001},
       URL = {https://doi.org/10.1016/j.jde.2021.07.001},
}


@article{paoli2021stability,
  AUTHOR = {Paoli, Gloria and Piscitelli, Gianpaolo and Sannipoli,
              Rossanno},
     TITLE = {A stability result for the {S}teklov {L}aplacian eigenvalue
              problem with a spherical obstacle},
   JOURNAL = {Commun. Pure Appl. Anal.},
  FJOURNAL = {Communications on Pure and Applied Analysis},
    VOLUME = {20},
      YEAR = {2021},
    NUMBER = {1},
     PAGES = {145--158},
      ISSN = {1534-0392,1553-5258},
   MRCLASS = {35J25 (28A75 35P15)},
  MRNUMBER = {4191500},
       DOI = {10.3934/cpaa.2020261},
       URL = {https://doi.org/10.3934/cpaa.2020261},
}


@article{makai1959principal,
  title={On the principal frequency of a convex membrane and related problems},
  author={Makai, Endre},
  journal={Czechoslovak Mathematical Journal},
  volume={9},
  number={1},
  pages={66--70},
  year={1959},
  publisher={Institute of Mathematics, Academy of Sciences of the Czech Republic}
}

@article{polya1960two,
  title={Two more inequalities between physical and geometrical quantities},
  author={P{\'o}lya, G},
  journal={J. Indian Math. Soc.(NS)},
  volume={24},
  number={1961},
  pages={413--419},
  year={1960}
}

@article{gavitone2021isoperimetric,
AUTHOR = {Gavitone, Nunzia and Paoli, Gloria and Piscitelli, Gianpaolo
              and Sannipoli, Rossano},
     TITLE = {An isoperimetric inequality for the first
              {S}teklov-{D}irichlet {L}aplacian eigenvalue of convex sets
              with a spherical hole},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {320},
      YEAR = {2022},
    NUMBER = {2},
     PAGES = {241--259},
      ISSN = {0030-8730,1945-5844},
   MRCLASS = {35P15 (28A75 35J25)},
  MRNUMBER = {4548311},
       DOI = {10.2140/pjm.2022.320.241},
       URL = {https://doi.org/10.2140/pjm.2022.320.241},
}

@article{hong2022first,
 AUTHOR = {Hong, Jiho and Lim, Mikyoung and Seo, Dong-Hwi},
     TITLE = {On the first {S}teklov-{D}irichlet eigenvalue for eccentric
              annuli},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {201},
      YEAR = {2022},
    NUMBER = {2},
     PAGES = {769--799},
      ISSN = {0373-3114,1618-1891},
   MRCLASS = {35P15 (49Q10 49Q12 49R05 65D99)},
  MRNUMBER = {4386844},
       DOI = {10.1007/s10231-021-01137-y},
       URL = {https://doi.org/10.1007/s10231-021-01137-y},
}

@article{gavitone2024monotonicity,
  AUTHOR = {Gavitone, Nunzia and Piscitelli, Gianpaolo},
     TITLE = {A monotonicity result for the first {S}teklov-{D}irichlet
              {L}aplacian eigenvalue},
   JOURNAL = {Rev. Mat. Complut.},
  FJOURNAL = {Revista Matem\'atica Complutense},
    VOLUME = {37},
      YEAR = {2024},
    NUMBER = {2},
     PAGES = {509--523},
      ISSN = {1139-1138,1988-2807},
   MRCLASS = {35J25 (28A75 35P15 49Q10 49R05)},
  MRNUMBER = {4739545},
MRREVIEWER = {Mihai\ Mih\u ailescu},
       DOI = {10.1007/s13163-023-00465-2},
       URL = {https://doi.org/10.1007/s13163-023-00465-2},
}


@article{barbato2023first,
  title={On the first {R}obin eigenvalue of the {F}insler $p$-{L}aplace operator as $p\to 1$},
  author={Barbato, Rosa and Della Pietra, Francesco and Piscitelli, Gianpaolo},
  journal={arXiv preprint arXiv:2301.01546},
  year={2023}
}
@article{gavitone2023steklov,
  AUTHOR = {Gavitone, Nunzia and Sannipoli, Rossano},
     TITLE = {On a {S}teklov-{R}obin eigenvalue problem},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {526},
      YEAR = {2023},
    NUMBER = {2},
     PAGES = {Paper No. 127254, 19},
      ISSN = {0022-247X,1096-0813},
   MRCLASS = {35P15},
  MRNUMBER = {4569253},
       DOI = {10.1016/j.jmaa.2023.127254},
       URL = {https://doi.org/10.1016/j.jmaa.2023.127254},
}


@article{hansen1994isoperimetric,
 AUTHOR = {Hansen, W. and Nadirashvili, N.},
     TITLE = {Isoperimetric inequalities in potential theory},
 BOOKTITLE = {Proceedings from the {I}nternational {C}onference on
              {P}otential {T}heory ({A}mersfoort, 1991)},
   JOURNAL = {Potential Anal.},
  FJOURNAL = {Potential Analysis. An International Journal Devoted to the
              Interactions between Potential Theory, Probability Theory,
              Geometry and Functional Analysis},
    VOLUME = {3},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {1--14},
      ISSN = {0926-2601,1572-929X},
   MRCLASS = {31A15 (31B15 35P15 52A40)},
  MRNUMBER = {1266215},
MRREVIEWER = {J.\ Hersch},
       DOI = {10.1007/BF01047833},
       URL = {https://doi.org/10.1007/BF01047833},
}


@article{melas1992stability,
  title={The stability of some eigenvalue estimates},
  author={Melas, Antonios D},
  journal={Journal of Differential Geometry},
  volume={36},
  number={1},
  pages={19--33},
  year={1992},
  publisher={Lehigh University}
}



@article{cianchi2008quantitative,
  title={A quantitative {P}{\'o}lya-{S}zeg{\"o} principle},
  author={Cianchi, Andrea and Esposito, Luca and Fusco, Nicola and Trombetti, Cristina},
  year={2008},
  journal={Journal für die reine und angewandte Mathematik},
  publisher={Walter de Gruyter}
}


@article{brasco2015faber,
  title={Faber--{K}rahn inequalities in sharp quantitative form},
  author={Brasco, Lorenzo and De Philippis, Guido and Velichkov, Bozhidar},
  journal={Duke Mathematical Journal},
  volume={164},
  number={9},
  pages={1777--1831},
  year={2015},
  publisher={Duke University Press}
}

@article{bhattacharya2001some,
  title={Some observations on the first eigenvalue of the $p$-{L}aplacian and its connections with asymmetry.},
  author={Bhattacharya, Tilak},
  journal={Electronic Journal of Differential Equations (EJDE)[electronic only]},
  volume={2001},
  pages={Paper--No},
  year={2001},
  publisher={Southwest Texas State University, Department of Mathematics, San Marcos, TX~…}
}

@article{fusco2009stability,
  title={Stability estimates for certain {F}aber-{K}rahn, isocapacitary and {C}heeger inequalities},
  author={Fusco, Nicola and Maggi, Francesco and Pratelli, Aldo},
  journal={Annali della Scuola Normale Superiore di Pisa-Classe di Scienze},
  volume={8},
  number={1},
  pages={51--71},
  year={2009}
}

@article{brasco2012sharp,
  title={Sharp stability of some spectral inequalities},
  author={Brasco, Lorenzo and Pratelli, Aldo},
  journal={Geometric and Functional Analysis},
  volume={22},
  number={1},
  pages={107--135},
  year={2012},
  publisher={Springer}
}


@article{cito2021quantitative,
   AUTHOR = {Cito, Simone and La Manna, Domenico Angelo},
     TITLE = {A quantitative reverse {F}aber-{K}rahn inequality for the
              first {R}obin eigenvalue with negative boundary parameter},
   JOURNAL = {ESAIM Control Optim. Calc. Var.},
  FJOURNAL = {ESAIM. Control, Optimisation and Calculus of Variations},
    VOLUME = {27},
      YEAR = {2021},
     PAGES = {Paper No. S23, 16},
      ISSN = {1292-8119,1262-3377},
   MRCLASS = {35P15 (35B35 49Q10 49R05)},
  MRNUMBER = {4222176},
       DOI = {10.1051/cocv/2020079},
       URL = {https://doi.org/10.1051/cocv/2020079},
}


@article{amato2024estimates,
    AUTHOR = {Amato, Vincenzo and Gentile, Andrea and Masiello, Alba Lia},
     TITLE = {Estimates for {R}obin {$p$}-{L}aplacian eigenvalues of convex
              sets with prescribed perimeter},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {533},
      YEAR = {2024},
    NUMBER = {2},
     PAGES = {Paper No. 128002, 20},
      ISSN = {0022-247X,1096-0813},
   MRCLASS = {35P05 (35J92 49J10 49R05)},
  MRNUMBER = {4682474},
MRREVIEWER = {Valeri\ S.\ Serov},
       DOI = {10.1016/j.jmaa.2023.128002},
       URL = {https://doi.org/10.1016/j.jmaa.2023.128002},
}
  

@article{brasco2012spectral,
 AUTHOR = {Brasco, Lorenzo and De Philippis, Guido and Ruffini, Berardo},
     TITLE = {Spectral optimization for the {S}tekloff-{L}aplacian: the
              stability issue},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {11},
     PAGES = {4675--4710},
      ISSN = {0022-1236,1096-0783},
   MRCLASS = {35P15 (35J05 35J20)},
  MRNUMBER = {2913683},
MRREVIEWER = {J.\ B.\ Kennedy},
       DOI = {10.1016/j.jfa.2012.03.017},
       URL = {https://doi.org/10.1016/j.jfa.2012.03.017},
}


@article{bucur2018quantitative,
  title={The quantitative {F}aber-{K}rahn inequality for the {R}obin {L}aplacian},
  author={Bucur, Dorin and Ferone, Vincenzo and Nitsch, Carlo and Trombetti, Cristina},
  journal={Journal of Differential Equations},
  volume={264},
  number={7},
  pages={4488--4503},
  year={2018},
  publisher={Elsevier}
}

@article {bfnt,
    AUTHOR = {Bucur, Dorin and Ferone, Vincenzo and Nitsch, Carlo and
              Trombetti, Cristina},
     TITLE = {A sharp estimate for the first {R}obin-{L}aplacian eigenvalue
              with negative boundary parameter},
   JOURNAL = {Atti Accad. Naz. Lincei Rend. Lincei Mat. Appl.},
  FJOURNAL = {Atti della Accademia Nazionale dei Lincei. Rendiconti Lincei.
              Matematica e Applicazioni},
    VOLUME = {30},
      YEAR = {2019},
    NUMBER = {4},
     PAGES = {665--676},
      ISSN = {1120-6330,1720-0768},
   MRCLASS = {35P15 (35J05 58J50)},
  MRNUMBER = {4030345},
MRREVIEWER = {Rodica\ Luca},
       DOI = {10.4171/RLM/866},
       URL = {https://doi.org/10.4171/RLM/866},
}




@article{gavitone2020quantitative,
  AUTHOR = {Gavitone, Nunzia and La Manna, Domenico Angelo and Paoli,
              Gloria and Trani, Leonardo},
     TITLE = {A quantitative {W}einstock inequality for convex sets},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {59},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {Paper No. 2, 20},
      ISSN = {0944-2669,1432-0835},
   MRCLASS = {35P15 (35B35 35J05)},
  MRNUMBER = {4037463},
MRREVIEWER = {Rodica\ Luca},
       DOI = {10.1007/s00526-019-1642-9},
       URL = {https://doi.org/10.1007/s00526-019-1642-9},
}

@article{bareket1977isoperimetric,
  title={On an isoperimetric inequality for the first eigenvalue of a boundary value problem},
  author={Bareket, Miriam},
  journal={SIAM Journal on Mathematical Analysis},
  volume={8},
  number={2},
  pages={280--287},
  year={1977},
  publisher={SIAM}
}


@article{ferone2015conjectured,
  AUTHOR = {Ferone, Vincenzo and Nitsch, Carlo and Trombetti, Cristina},
     TITLE = {On a conjectured reverse {F}aber-{K}rahn inequality for a
              {S}teklov-type {L}aplacian eigenvalue},
   JOURNAL = {Commun. Pure Appl. Anal.},
  FJOURNAL = {Communications on Pure and Applied Analysis},
    VOLUME = {14},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {63--82},
      ISSN = {1534-0392,1553-5258},
   MRCLASS = {35P15 (28A75 35J05 35J20 46E35 49Q10)},
  MRNUMBER = {3299025},
MRREVIEWER = {Kazuhiro\ Kurata},
       DOI = {10.3934/cpaa.2015.14.63},
       URL = {https://doi.org/10.3934/cpaa.2015.14.63},
}


@article{freitas2015first,
  title={The first {R}obin eigenvalue with negative boundary parameter},
  author={Freitas, Pedro and Krej{\v{c}}i{\v{r}}{\'\i}k, David},
  journal={Advances in Mathematics},
  volume={280},
  pages={322--339},
  year={2015},
  publisher={Elsevier}
}

@article{kovavrik2017p,
  title={On the p-{L}aplacian with {R}obin boundary conditions and boundary trace theorems},
  author={Kova{\v{r}}{\'\i}k, Hynek and Pankrashkin, Konstantin},
  journal={Calculus of Variations and Partial Differential Equations},
  volume={56},
  number={2},
  pages={1--29},
  year={2017},
  publisher={Springer}
}

@article{fuglede1989stability,
  AUTHOR = {Fuglede, Bent},
     TITLE = {Stability in the isoperimetric problem for convex or nearly
              spherical domains in {${\bf R}^n$}},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {314},
      YEAR = {1989},
    NUMBER = {2},
     PAGES = {619--638},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {52A40},
  MRNUMBER = {942426},
MRREVIEWER = {Catherine\ Bandle},
       DOI = {10.2307/2001401},
       URL = {https://doi.org/10.2307/2001401},
}

@article{fusco2015quantitative,
  AUTHOR = {Fusco, Nicola},
     TITLE = {The quantitative isoperimetric inequality and related topics},
   JOURNAL = {Bull. Math. Sci.},
  FJOURNAL = {Bulletin of Mathematical Sciences},
    VOLUME = {5},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {517--607},
      ISSN = {1664-3607,1664-3615},
   MRCLASS = {49Q20 (28A75 52A40 53A10)},
  MRNUMBER = {3404715},
MRREVIEWER = {Georgios\ Psaradakis},
       DOI = {10.1007/s13373-015-0074-x},
       URL = {https://doi.org/10.1007/s13373-015-0074-x},
}

@book{watson1922theory,
  title={Theory of {B}essel functions},
  author={Watson, George Neville},
  volume={3},
  year={1922},
  publisher={The University Press}
}


@article{verma2020eigenvalue,
 AUTHOR = {Verma, Sheela and Santhanam, G.},
     TITLE = {On eigenvalue problems related to the laplacian in a class of
              doubly connected domains},
   JOURNAL = {Monatsh. Math.},
  FJOURNAL = {Monatshefte f\"ur Mathematik},
    VOLUME = {193},
      YEAR = {2020},
    NUMBER = {4},
     PAGES = {879--899},
      ISSN = {0026-9255,1436-5081},
   MRCLASS = {35P15 (35J05 58J50)},
  MRNUMBER = {4159863},
       DOI = {10.1007/s00605-020-01466-9},
       URL = {https://doi.org/10.1007/s00605-020-01466-9},
}

@article {AGM,
    AUTHOR = {Amato, Vincenzo and Gentile, Andrea and Masiello, Alba Lia},
     TITLE = {Comparison results for solutions to {$p$}-{L}aplace equations
              with {R}obin boundary conditions},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {201},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {1189--1212},
      ISSN = {0373-3114},
   MRCLASS = {35J92 (35P15)},
  MRNUMBER = {4426282},
       DOI = {10.1007/s10231-021-01153-y},
       URL = {https://doi.org/10.1007/s10231-021-01153-y},
}

@incollection {talenti,
    AUTHOR = {Talenti, Giorgio},
     TITLE = {The standard isoperimetric theorem},
 BOOKTITLE = {Handbook of convex geometry, {V}ol. {A}, {B}},
     PAGES = {73--123},
 PUBLISHER = {North-Holland, Amsterdam},
      YEAR = {1993},
   MRCLASS = {49Q10 (49-02 52A40)},
  MRNUMBER = {1242977},
MRREVIEWER = {Harold Parks},
       DOI = {10.1016/B978-0-444-89596-7.50008-0},
       URL = {https://doi.org/10.1016/B978-0-444-89596-7.50008-0},
}
@book {chavel,
    AUTHOR = {Chavel, Isaac},
     TITLE = {Isoperimetric inequalities},
    SERIES = {Cambridge Tracts in Mathematics},
    VOLUME = {145},
      NOTE = {Differential geometric and analytic perspectives},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2001},
     PAGES = {xii+268},
      ISBN = {0-521-80267-9},
   MRCLASS = {58J35 (35B05 49Q15 53C20 58-02)},
  MRNUMBER = {1849187},
MRREVIEWER = {Thierry Coulhon},
}

@article{ftouhi2022place,
   AUTHOR = {Ftouhi, Ilias},
     TITLE = {Where to place a spherical obstacle so as to maximize the
              first nonzero {S}teklov eigenvalue},
   JOURNAL = {ESAIM Control Optim. Calc. Var.},
  FJOURNAL = {ESAIM. Control, Optimisation and Calculus of Variations},
    VOLUME = {28},
      YEAR = {2022},
     PAGES = {Paper No. 6, 21},
      ISSN = {1292-8119,1262-3377},
   MRCLASS = {49R05 (35P05 49Q10)},
  MRNUMBER = {4364336},
MRREVIEWER = {Mrityunjoy\ Ghosh},
       DOI = {10.1051/cocv/2021109},
       URL = {https://doi.org/10.1051/cocv/2021109},
}

@article{biswas2021optimization, 
AUTHOR = {Biswas, Nirjan and Das, Ujjal and Ghosh, Mrityunjoy},
     TITLE = {On the optimization of the first weighted eigenvalue},
   JOURNAL = {Proc. Roy. Soc. Edinburgh Sect. A},
  FJOURNAL = {Proceedings of the Royal Society of Edinburgh. Section A.
              Mathematics},
    VOLUME = {153},
      YEAR = {2023},
    NUMBER = {6},
     PAGES = {1777--1804},
      ISSN = {0308-2105,1473-7124},
   MRCLASS = {35P15 (35B06 35J92 49J30 49R05)},
  MRNUMBER = {4666058},
MRREVIEWER = {Stefan\ Steinerberger},
       DOI = {10.1017/prm.2022.60},
       URL = {https://doi.org/10.1017/prm.2022.60},
}

@article{chorwadwala2022optimal,
   AUTHOR = {Chorwadwala, Anisa M. H. and Ghosh, Mrityunjoy},
     TITLE = {Optimal shapes for the first {D}irichlet eigenvalue of the
              {$p$}-{L}aplacian and dihedral symmetry},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {508},
      YEAR = {2022},
    NUMBER = {2},
     PAGES = {Paper No. 125901, 18},
      ISSN = {0022-247X,1096-0813},
   MRCLASS = {49R05 (35P30 49Q10)},
  MRNUMBER = {4353251},
MRREVIEWER = {Patrik\ Knopf},
       DOI = {10.1016/j.jmaa.2021.125901},
       URL = {https://doi.org/10.1016/j.jmaa.2021.125901},
}

@article{amato2023talenti,
  title={The {T}alenti comparison result in a quantitative form},
  author={Amato, Vincenzo and Barbato, Rosa and Masiello, Alba Lia and Paoli, Gloria},
  journal={Annali della Scuola Normale Superiore di Pisa-Classe di Scienze},
  year={2024},
   Doi={https://doi.org/10.2422/2036-2145.202404_010},
volume={31}
}

@article {citogiaco,
    AUTHOR = {Cito, Simone and Giacomini, Alessandro},
     TITLE = {Minimization of the {$k$}-th eigenvalue of the
              {R}obin-{L}aplacian with perimeter constraint},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {63},
      YEAR = {2024},
    NUMBER = {9},
     PAGES = {Paper No. 244, 38},
      ISSN = {0944-2669,1432-0835},
   MRCLASS = {49R05 (26B30 35J20 35P05 35R35 49J35 49J45 49Q10)},
  MRNUMBER = {4824702},
       DOI = {10.1007/s00526-024-02872-9},
       URL = {https://doi.org/10.1007/s00526-024-02872-9},
}

@article {AMaRo,
    AUTHOR = {Andreu, F. and Maz\'on, J. M. and Rossi, J. D.},
     TITLE = {The best constant for the {S}obolev trace embedding from
              {$W^{1,1}(\Omega)$} into {$L^1(\partial\Omega)$}},
   JOURNAL = {Nonlinear Anal.},
  FJOURNAL = {Nonlinear Analysis. Theory, Methods \& Applications. An
              International Multidisciplinary Journal},
    VOLUME = {59},
      YEAR = {2004},
    NUMBER = {7},
     PAGES = {1125--1145},
      ISSN = {0362-546X,1873-5215},
   MRCLASS = {35J60 (26D15 35J20 46E35)},
  MRNUMBER = {2098509},
MRREVIEWER = {Eduardo\ Colorado},
       DOI = {10.1016/j.na.2004.07.051},
       URL = {https://doi.org/10.1016/j.na.2004.07.051},
}

@book {AFP,
    AUTHOR = {Ambrosio, Luigi and Fusco, Nicola and Pallara, Diego},
     TITLE = {Functions of bounded variation and free discontinuity
              problems},
    SERIES = {Oxford Mathematical Monographs},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {2000},
     PAGES = {xviii+434},
      ISBN = {0-19-850245-1},
   MRCLASS = {49-02 (49J45 49K10 49Qxx)},
  MRNUMBER = {1857292},
MRREVIEWER = {J.\ E.\ Brothers},
}

@article{DoTo,
AUTHOR = {Lami Dozo, Enrique J. and Torn\'e, Olaf},
     TITLE = {Symmetry and symmetry breaking for minimizers in the trace
              inequality},
   JOURNAL = {Commun. Contemp. Math.},
  FJOURNAL = {Communications in Contemporary Mathematics},
    VOLUME = {7},
      YEAR = {2005},
    NUMBER = {6},
     PAGES = {727--746},
      ISSN = {0219-1997,1793-6683},
   MRCLASS = {35J20 (26D15 35A30 35J60 47J30)},
  MRNUMBER = {2193239},
MRREVIEWER = {Marco\ Squassina},
       DOI = {10.1142/S0219199705001921},
       URL = {https://doi.org/10.1142/S0219199705001921},
}

@article {cclp,
    AUTHOR = {Carbotti, Alessandro and Cito, Simone and La Manna, Domenico
              Angelo and Pallara, Diego},
     TITLE = {A quantitative dimension free isoperimetric inequality for the
              fractional {G}aussian perimeter},
   JOURNAL = {Comm. Anal. Geom.},
  FJOURNAL = {Communications in Analysis and Geometry},
    VOLUME = {32},
      YEAR = {2024},
    NUMBER = {2},
     PAGES = {577--603},
      ISSN = {1019-8385,1944-9992},
   MRCLASS = {49Q15 (49Q20)},
  MRNUMBER = {4828192},
       DOI = {10.4310/cag.241015013216},
       URL = {https://doi.org/10.4310/cag.241015013216},
}


@article {cclp2,
    AUTHOR = {Carbotti, Alessandro and Cito, Simone and La Manna, Domenico
              Angelo and Pallara, Diego},
     TITLE = {Stability of the {G}aussian {F}aber-{K}rahn inequality},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {203},
      YEAR = {2024},
    NUMBER = {5},
     PAGES = {2185--2198},
      ISSN = {0373-3114,1618-1891},
   MRCLASS = {35P15 (49Q10 49R05)},
  MRNUMBER = {4797290},
MRREVIEWER = {Yunfeng\ Shi},
       DOI = {10.1007/s10231-024-01441-3},
       URL = {https://doi.org/10.1007/s10231-024-01441-3},
}




@article{cpp2,
author = {Cito, Simone and Paoli, Gloria and Piscitelli, Gianpaolo},
title = {A quantitative Payne-Weinberger type inequality},
journal = {IN PROGRESS},
}

@article{bugitr,
title = {Best constant in {P}oincaré inequalities with traces: A free discontinuity approach},
journal = {Annales de l'Institut Henri Poincaré C, Analyse non linéaire},
volume = {36},
number = {7},
pages = {1959-1986},
year = {2019},
issn = {0294-1449},
doi = {https://doi.org/10.1016/j.anihpc.2019.07.007},
url = {https://www.sciencedirect.com/science/article/pii/S0294144919300812},
author = {Dorin Bucur and Alessandro Giacomini and Paola Trebeschi},
}

@article{bugitr16,
	 AUTHOR = {Bucur, Dorin and Giacomini, Alessandro and Trebeschi, Paola},
     TITLE = {The {R}obin-{L}aplacian problem on varying domains},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {55},
      YEAR = {2016},
    NUMBER = {6},
     PAGES = {Art. 133, 29},
      ISSN = {0944-2669,1432-0835},
   MRCLASS = {35J25 (26A45 35B35 35J20 47J30)},
  MRNUMBER = {3566212},
MRREVIEWER = {Vicen\c tiu\ D.\ R\u adulescu},
       DOI = {10.1007/s00526-016-1073-9},
       URL = {https://doi.org/10.1007/s00526-016-1073-9},
}


@article{bragonisp,
author = {Brasco, L. and Gonz\'{a}lez, M. and Ispizua, M.},
title = {A {S}teklov version of the torsional rigidity},
journal = {Communications in Contemporary Mathematics},
volume = {26},
number = {07},
pages = {2350037},
year = {2024},
doi = {10.1142/S0219199723500372},

URL = {    
        https://doi.org/10.1142/S0219199723500372
},
eprint = {    
        https://doi.org/10.1142/S0219199723500372
}}

@article{massal,
AUTHOR = {Masiello, Alba Lia and Salerno, Francesco},
     TITLE = {A quantitative result for the {$k$}-{H}essian equation},
   JOURNAL = {Nonlinear Anal.},
  FJOURNAL = {Nonlinear Analysis. Theory, Methods \& Applications. An
              International Multidisciplinary Journal},
    VOLUME = {255},
      YEAR = {2025},
     PAGES = {Paper No. 113776, 16},
      ISSN = {0362-546X,1873-5215},
   MRCLASS = {52A39 (35B35 35J60 35J96)},
  MRNUMBER = {4867241},
       DOI = {10.1016/j.na.2025.113776},
       URL = {https://doi.org/10.1016/j.na.2025.113776},
}

@incollection {bdph,
    AUTHOR = {Brasco, Lorenzo and De Philippis, Guido},
     TITLE = {Spectral inequalities in quantitative form},
 BOOKTITLE = {Shape optimization and spectral theory},
     PAGES = {201--281},
 PUBLISHER = {De Gruyter Open, Warsaw},
      YEAR = {2017},
      ISBN = {978-3-11-055088-7; 978-3-11-055085-6},
   MRCLASS = {58J50 (58J32)},
  MRNUMBER = {3681151},
MRREVIEWER = {Juan\ Manuel\ P\'erez-Pardo},
       DOI = {10.1515/9783110550887-007},
       URL = {https://doi.org/10.1515/9783110550887-007},
}

@article {BGR,
    AUTHOR = {Bonder, Juli\'an Fern\'andez and Groisman, Pablo and Rossi,
              Julio D.},
     TITLE = {Optimization of the first {S}teklov eigenvalue in domains with
              holes: a shape derivative approach},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {186},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {341--358},
      ISSN = {0373-3114,1618-1891},
   MRCLASS = {35P15 (35J05 35J25 49Q10 58J50)},
  MRNUMBER = {2295124},
MRREVIEWER = {Julian\ Edward},
       DOI = {10.1007/s10231-006-0009-y},
       URL = {https://doi.org/10.1007/s10231-006-0009-y},
}


@article {grosch,
    AUTHOR = {Groemer, H. and Schneider, R.},
     TITLE = {Stability estimates for some geometric inequalities},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {23},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {67--74},
      ISSN = {0024-6093,1469-2120},
   MRCLASS = {52A40 (52A38)},
  MRNUMBER = {1111537},
MRREVIEWER = {P.\ R.\ Goodey},
       DOI = {10.1112/blms/23.1.67},
       URL = {https://doi.org/10.1112/blms/23.1.67},
}

@article{barbato2025talenticomparisonresultssolutions,
      title={Talenti comparison results for solutions to $p$-{L}aplace equation on multiply connected domains}, 
      author={Luca Barbato and Francesco Salerno},
 journal={arXiv preprint arXiv:2504.06103},
      year={2025},
      eprint={2504.06103},
      archivePrefix={arXiv},
      primaryClass={math.AP},
      url={https://arxiv.org/abs/2504.06103}, 
}

@article {lasan,
    AUTHOR = {La Manna, Domenico Angelo and Sannipoli, Rossano},
     TITLE = {Some isoperimetric inequalities involving the boundary
              momentum},
   JOURNAL = {J. Optim. Theory Appl.},
  FJOURNAL = {Journal of Optimization Theory and Applications},
    VOLUME = {207},
      YEAR = {2025},
    NUMBER = {2},
     PAGES = {Paper No. 32, 36},
      ISSN = {0022-3239,1573-2878},
   MRCLASS = {49Q10 (26D10 26D20)},
  MRNUMBER = {4938969},
       DOI = {10.1007/s10957-025-02757-7},
       URL = {https://doi.org/10.1007/s10957-025-02757-7},
}

@misc{amabar,
      title={On the stability of the annulus for the torsion of multiply connected domains}, 
      author={Vincenzo Amato and Luca Barbato},
      year={2025},
      eprint={2506.07592},
      archivePrefix={arXiv},
      primaryClass={math.AP},
      url={https://arxiv.org/abs/2506.07592}, 
}
